Understanding Fixed Predictions via Confined Regions

Machine learning models can assign fixed predictions that preclude individuals from changing their outcome. Existing approaches to audit fixed predictions do so on a pointwise basis, which requires access to an existing dataset of individuals and may fail to anticipate fixed predictions in out-of-sample data. This work presents a new paradigm to identify fixed predictions by finding confined regions of the feature space in which all individuals receive fixed predictions. This paradigm enables the certification of recourse for out-of-sample data, works in settings without representative datasets, and provides interpretable descriptions of individuals with fixed predictions. We develop a fast method to discover confined regions for linear classifiers using mixed-integer quadratically constrained programming. We conduct a comprehensive empirical study of confined regions across diverse applications. Our results highlight that existing pointwise verification methods fail to anticipate future individuals with fixed predictions, while our method both identifies them and provides an interpretable description.

==> deprecated/1_introduction.tex <==
\section{Introduction}

Machine Learning is increasingly used in high-stakes settings to decide who receives a loan \citep{hurley2016credit}, a job interview~\citep{bogen2018help}, or even organ transplants ~\citep{murgia2023algorithms}. Models are designed to predict outcomes using features about individuals, but fail to take into account constraints on how individuals can change them~\citep[][]{liu2024actionability}. Consequently, models may assign an individual a \emph{fixed prediction} which is not \emph{responsive} to the individual's actions.

The responsiveness of a model is integral to its safety in settings where predictions map to people. In domains such as healthcare, recent results have highlighted how young patients may be inadvertently precluded from receiving a liver transplant as a result fixed predictions~\cite{murgia2023algorithms}. In settings like content moderation, a fixed prediction can ensure that malicious actors are unable to evade detection by manipulating their features. %Across these settings, it is vital to understand what individuals do not have \emph{recourse}, the ability to change the decision of the model through their actions. %Before deploying a model, it is critical that stakeholders understand and characterize what individuals affected by their model are precluded from receiving a desirable outcome. 

In this paper, we study the problem of understanding whether any individuals are assigned a fixed prediction in an \emph{entire region} of the feature space (e.g., all plausible job applicants). 
While prior work has focused on verifying the existence of recourse for individuals, these individualized approaches do not provide any guarantees on the responsiveness of the model for out-of-sample data. In settings like lending and hiring, this means that critical issues can only be identified \emph{after} a model has been deployed. Moreover, even when individuals without recourse can be identified during model development, determining the root cause of fixed predictions can be challenging. Recent work has highlighted that individualized recourse approaches alone are insufficient to facilitate broader model understanding and debugging~\citep{rawal2020algorithmic}. Auditing the responsiveness of a model with individualized approaches requires access to a representative dataset of individuals affected by the model. This requirement is demanding for external audits where gaining access to a model is easy but getting a representative sample of the population is difficult. For instance, many interpretable medical and criminal justice scoring systems are available publicly~\citep[see e.g.,][]{morrison2022optimized, yamga2023optimized, ribeiro2023use, PennSentence}, but gaining access to a representative dataset is difficult due to privacy concerns. %Here, external auditors are either have to rely on small datasets to audit responsiveness or try to create representative synthetic datasets. 

In response to these challenges, we introduce a new tool to verify recourse over a region of the feature space. We do so for linear classification models, a broad function class encompassing popular methods such as logistic regression, linearizable rule-based models (e.g., rule sets, decision lists), and concept-bottleneck models \cite{koh2020concept, sun2024concept}. Previous work has highlighted that recourse verification for a \emph{single individual} is a non-trivial combinatorial problem that requires performing exhaustive search over a subset of the feature space that captures both the model as well as actionability constraints \cite{ustun2019actionable, kothari2023prediction}. Our approach generalizes this problem to an even more intensive setting that requires searching over an entire region of individuals. Despite these challenges, our approach is able to verify recourse over regions within seconds on real-world datasets. Moreover, our tool is designed to find \emph{static regions} within the feature space (i.e., regions where individuals are assigned a fixed prediction), which can help model developers determine the root causes of fixed predictions. Our tool can be run in settings without a public dataset, enabling practitioners to audit model responsiveness with only access to the model itself and a description of the region on which it is being deployed. 

%This work studies a new paradigm in algorithmic recourse that aims to characterize fixed predictions.% by verifying recourse over an \emph{entire region} of the feature space (e.g., all plausible job applicants). 
%We introduce a new tool that formally verifies recourse over an \emph{entire region} of the feature space (e.g., all plausible job applicants). Our tool can be used to discover interpretable \emph{static regions} (i.e., where all individuals are assigned a fixed prediction) within this space, or provide a formal certification of model responsiveness over the entire region. Our approach is robust to distribution shifts and runs in seconds on real-world datasets.  Moreover, our tool can be used without the need for available datasets, enabling practitioners to audit model responsiveness in settings with only model access and a description of the region on which it is being deployed. For instance, many interpretable medical and criminal justice scoring systems are available publicly~\citep[see e.g.,][]{morrison2022optimized, yamga2023optimized, ribeiro2023use, PennSentence}, but gaining access to a representative dataset is difficult due to privacy concerns. 

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/overview_figure.pdf}
    \vspace{-3em}
    \caption{Sample recourse verification task over a region. The feature space contains a continuous feature \textds{Years of Experience (YoE)}, and a binary feature \textds{Male} that encodes gender. We denote actions on each feature ($a_{\textds{YoE}}, a_{\textds{Male}}$) and specify constraints on feasible actions in the \emph{action set}. The task is to verify the responsiveness of a linear classifier over a \emph{region}, an area of the feature space defined by a set of constraints. Under this classifier there exists a \emph{static region}, an area where all applicants are assigned a fixed prediction. }
    \label{fig:summary}
    \vspace{-1em}
\end{figure*}

The main contributions of this work include:
\begin{enumerate}[leftmargin=*,itemsep=0]
    % Conceptual Contributions
    \item We introduce a new approach to formally verify recourse for linear classifiers over entire regions of the feature space. This tool can be used certify the responsiveness of classifiers beyond data present in a training dataset and can provide stronger guarantees for out-of-sample data. We also present tools to find (or enumerate all) static regions in the feature space, providing an intuitive tool for model developers to audit and correct problems with model responsiveness.

    % Method Constribution
    \item We develop fast methods that are able to find static regions within the feature space via Mixed-Integer Quadratically Constrained Programming (MIQCP). Our approach handles a broad class of actionability constraints, and can verify recourse within seconds on real-world datasets.
    
    % Empirical Contribution
    \item We evaluate our approach on applications in consumer finance, content moderation, and criminal justice. Our results show that existing approaches fail to verify model responsiveness over regions, emphasizing the need for tools that audit recourse beyond individual data points. We also showcase the ability of our approach to audit model responsiveness in settings with no public datasets via a case-study on the Pennsylvania criminal justice sentencing risk assessment instrument.


    % Software
    %\item We include a Python implementation of our approach that builds upon existing APIs for actionable recourse, allowing practitioners to easily specify complex actionability constraints and audit recourse.
    
\end{enumerate}




==> deprecated/3_problem_setup_old.tex <==
\section{Recourse Verification over Populations}
We consider a binary classification task where the goal is to predict a label $y \in \{0,1\}$ from a set of $d$ features $\mathbf{x} = [x_1, x_2, \dots, x_d ] \in {\cal X}$ where ${\cal X} \subseteq \mathbb{R}^{d+1}$ is a bounded set representing a population of individuals. We assume that the population ${\cal X}$ can be represented by a set of linear constraints over a mixed-integer set (see Fig. X for an example). This is an incredibly general assumption that encompasses a variety of potential populations ranging from regions as simple as a box to complex disjunctions over the convex hulls of different clusters of data. Throughout this paper we use boldface variables (e.g., $\mathbf{x}$) to denote vectors, and standard text with subscripts (e.g., $x_d$) to denote a specific element of a vector. We assume we have access to a linear classifier $f(x) = \text{sign}(\mathbf{w}^T\mathbf{x} + b)$ where $\mathbf{w} \in \mathbb{R}^d$ is a vector of coefficients and $b \in \mathbb{R}$ is the intercept of the classifier. Without loss of generality, we assume $f(x) = 1$ is the desired outcome (e.g., receiving a loan or job interview).

The recourse verification problem \cite{kothari2023prediction} tests whether an individual $\mathbf{x}$ can obtain the desired outcome of a model by changing their features, which we call \textit{actions}. Each action is a vector $\mathbf{a} \in \mathbb{R}^{d}$ that shifts the features of the individual to $\mathbf{x} + \mathbf{a} = \mathbf{x}' \in {\cal X}'$. We refer to the set of all actions an individual $\mathbf{x}$ can take as the \emph{action set} $A(\mathbf{x})$. In practice, an action set is represented by a set of constraints ~\citep[see][for details]{kothari2023prediction}. Note that in our setting, the population of potential individuals after taking an action ${\cal X}'$ may be different than the original population. For instance, we may want to verify recourse for individuals coming from a sub-population within a larger dataset (e.g., job applicants under 18 years old), but only want to constrain that the resulting feature vector is within the original population (e.g., resembles a realistic job application). We denote the \emph{recourse set} $R(x,f, A) = \{a: f(x + a) = 1, a \in A(x)\}$ as the set of feasible actions for an individual $x$ that lead to the desired outcome.

We study the problem of verifying recourse over the entire population of individuals ${\cal X}$. Formally, given a population ${\cal X}$, a classifier $f$, and a set of actionability constraints ${\cal A}$, the \textit{Population Recourse Verification Problem (PRVP) } checks whether there $\exists x \in {\cal X}: R(x, f, A) = \emptyset$. Note that this generalizes the recourse verification problem introduced in \citet{kothari2023prediction} to operate on an entire population of individuals. 

As a decision problem, the PRVP returns a yes or no response to whether a region has recourse. This binary response can make it difficult for model developers to interpret the root cause of the preclusion. To enhance interpretability, we also study an optimization variant of the PRVP that aims to find the largest region within the population without recourse. We focus on \textit{box} regions that are defined by simple upper and lower bound constraints on each feature. Let $U_j = \max_{x \in {\cal X}}x_j$, $L_j = \min_{x \in {\cal X}}x_j$ be the upper and lower bound for each feature $j$ in the population. Formally, for a given upper bound, $\mathbf{u} \in \mathbb{R}^d: \mathbf{u} \leq \mathbf{U}$, and lower bound, $\mathbf{l} \in \mathbb{R}^d: \mathbf{l} \leq \mathbf{L}$, a box region $B_{\cal X}(\mathbf{u},\mathbf{l})$ is defined as:
$$
B_{\cal X}(\mathbf{u},\mathbf{l}) = \{\mathbf{x} \in {\cal X}: \mathbf{l} \leq x \leq \mathbf{u}\}
$$
Box regions can be viewed as a decision rule (i.e., equivalent to the leaf node of a decision tree), which have been widely studied for their interpretability within the broader ML community (e.g., \cite{lawless2023interpretable, lawless2022interpretable, lawless2023cluster}).
For ease of notation we drop the explicit dependence on ${\cal X}$ and refer to box regions as $B(\mathbf{u}, \mathbf{l})$.
Note that setting $u_j = U_j$ ($l_j = L_j$) is equivalent to enforcing no upper bound (lower bound) on $x$ for feature $j$, and thus we can often express box regions with a small number of non-trivial constraints. We define the size of a box region $B(\mathbf{u},\mathbf{l})$ as the sum of the normalized ranges of each feature. Formally, the size of a region $B(\mathbf{u},\mathbf{l})$ is: $$\text{Size}(B(\mathbf{u}, \mathbf{l})) = \sum_{j=1}^d \frac{u_j - l_j}{U_j - L_j}$$ Note that this value is bounded between $0$ and $d$. We experimented with maximizing the area of the box (i.e., use a product instead of a sum) but found it to be much more computationally demanding empirically due to its non-linearity. In practice, we also found that maximizing the normalized range produced \emph{sparse} regions where only a few features were adjusted from their upper and lower bounds.

Given a population ${\cal X}$, a classifier $f$, and action set $A$, the \textit{Interpretable} PRVP aims to solve the following optimization problem:
\begin{align*}
\begin{split}
        \max\quad& \text{Size}(B(\mathbf{u}, \mathbf{l}))\\
        \textnormal{s.t.}\quad & \forall x \in B(\mathbf{u}, \mathbf{l}): R(x, f, A) = \emptyset\\
        & \mathbf{L} \leq \mathbf{l} \leq \mathbf{u} \leq \mathbf{U}
\end{split}
\end{align*}

Note that the output of the interpretable PRVP can be used to provide solutions to the original PRVP. For instance, the PVRP problem is a no-instance (i.e., certifies recourse for the entire population) if and only if the Interpretable PRVP is infeasible. Note that if the optimal value of the Interpretable PRVP $\text{Size}(B(\mathbf{u}^*, \mathbf{l}^*)) = \text{Size}(B(\mathbf{U}, \mathbf{L}))$ then the entire population has no recourse and is precluded from receiving the desirable outcome. We can also add additional constraints on the problem to answer other related questions. For instance, by constraining $\mathbf{u} = \mathbf{l}$ the PRVP will return a single data point within a population without recourse. 

\textbf{Use Cases:} Population-level recourse verification can be used in similar contexts as individualized recourse verification but provides stronger guarantees for out-of-sample deployment. %Moreover, identifying interpretable regions of preclusion can also aid in model development.

\emph{Detecting Preclusion.} In applications like lending and hiring where ML models need to safeguard against preclusion, our tools can be used to certify that all individuals in the population have recourse. Unlike existing approaches, these guarantees hold for out-of-sample data and can guarantee the absence of preclusion within the population on which a ML model is being deployed. 

\emph{Certifying Robustness.} Our approach can also certify the lack of recourse over a population, providing strong guarantees on model robustness to adversarial perturbations. For instance, in content moderation our tools can formally verify that malicious messages cannot bypass a filter by gaming their features. 

\emph{Characterizing Preclusion.} By iteratively using our tool to generate regions without recourse, our approach can enumerate precluded regions within a population. These regions are simple to understand and can be used to help debug ML models or provide a high-level summary of preclusion for stakeholders. 


%\textbf{Why is this task challenging?} A natural approach to auditing recourse over a population would be to verify the recourse of the worst-case member of the population (i.e., the individual $\mathbf{x}$ with the lowest score $\mathbf{w}^{\top} \mathbf{x}$). However, under complex actionability constraints there may be precluded individuals in the interior of the population --- even when the worst-case member has recourse (see Fig. X for an example). Therefore, heuristics that verify recourse for the worst-case member of the population cannot \emph{certify} recourse over the entire population.

%Therefore to \emph{formally certify} recourse over the population, individualized approaches would need to audit the recourse of every individual!

%connor{A corollary of our TUM result is that under linear recourse actionability constraints, if a population has an individual without recourse it'll be at \textit{an} extreme point. }



==> deprecated/4_ip_formulation.tex <==
\section{Verification via MIQCP} \label{sec:method}
Towards formally verifying recourse over an entire population, we formulate a MIQCP to solve the interpretable PRVP. We start by formulating the related problem of auditing whether a fixed region $B(\mathbf{u}, \mathbf{l})$ contains any data points with recourse, which we denote the \emph{Population Recourse Existence Problem (PREP)}. 

Let $\mathbf{x} \in \mathbb{R}^{d-m} \times \mathbb{Z}^m$ be a decision variable representing an  point, and $\mathbf{a} \in \mathbb{R}^{d-m} \times \mathbb{Z}^m$ represent an action. We formulate the PREP as a mixed-integer linear program (MILP) (see Appendix \ref{app:prep_form} for details). For ease of presentation, we summarize the PREP MILP formulation using the following standard form:
$$
A\mathbf{x} + B\mathbf{a} \leq b(\mathbf{u}, \mathbf{l})
$$
where $A$ and $B$ are $m \times d$ matrices and $b(u,l)$ is a $m$-dimensional vector that is a linear function of the box region upper and lower bounds $\mathbf{u}, \mathbf{l}$. Here $m$ represents the number of constraints in the full PREP.

Our goal is to find a region $B(\mathbf{u}, \mathbf{l})$ where no data points have recourse, and thus the PREP is infeasible. We start by considering the \emph{linear relaxation} of the problem that relaxes all integer variables to be continuous, which we denote as the \emph{Linear} PREP (L-PREP). To formulate the problem of finding $B(u, l)$ we leverage a classical result from linear optimization called Farkas' lemma: 

\begin{theorem}[\citet{farkas}]
Let $A \in \mathbb{R}^{m \times n}$ and $b \in \mathbb{R}^m$. Then exactly one of the following two assertions is true:
\begin{itemize}
    \item There exists $x \in \mathbb{R}^n$ such that $Ax \leq b$
    \item There exists $y \geq 0$ such that $A^T y = 0$ and $b^T y = -1$
\end{itemize}
\end{theorem}

Farkas' lemma states that we can certify that a system of inequalities $Ax \leq b$ is infeasible by finding a certificate $y \geq 0$ such that $A^\top y = 0$ and $b^\top y = -1$. In our context, we can thus view the problem of finding a region without recourse as a joint problem of selecting a region and ensuring there is an associated certificate of infeasibility for the L-PREP. 

Let $y \in \mathbb{R}^{m}$ be decision variables representing the certificate of infeasibility.  Note that there is one variable for every constraint in the original problem. We can now find the largest region $B(u, l)$ with associated certificate of infeasibility $y$ for the L-PREP using the following MIQCP formulation, which we denote the \emph{Linear PRVP (L-PRVP)}:

\begin{align}
	\textbf{max}~~&& \sum_d \frac{u_d - l_d}{U_d - L_d} \label{obj:size}\\[.1cm]
	\textbf{s.t.}~~&& b(\mathbf{u}, \mathbf{l})^T \mathbf{y} &= -1 ~~&& \label{const:neg_ray}\\
	&& A^T \mathbf{y} &= 0 && \label{const:dual_feas_a} \\
	&& B^T \mathbf{y} &= 0 && \label{const:dual_feas_b} \\
	&& \mathbf{y} &\geq 0 && \label{const:non_neg_y} \\
	&& \mathbf{L} \leq \mathbf{l} \leq \mathbf{u} &\leq \mathbf{U} && \label{const:box_bounds} \\
	&& \mathbf{u}, \mathbf{l} &\in \mathbb{Z}^d \label{const:ul_int}
\end{align}

The objective of the problem is to maximize the size of $B(\mathbf{u}, \mathbf{l})$. Constraints \eqref{const:neg_ray}-\eqref{const:non_neg_y} follow from Farkas' lemma and ensure that $y$ is a valid certificate of infeasibility for the linear relaxation of the PREP. Constraints \eqref{const:box_bounds} and \eqref{const:ul_int} ensure we generate a valid region $B(\mathbf{u}, \mathbf{l})$. We restrict $\mathbf{u}, \mathbf{l}$ to be integer variables to prevent numerical precision issues when solving the MIQCP. This is not an onerous assumption as any continuous variable $x_j$ with a desired precision $10^{-p}$ can be re-scaled and rounded to an integer variable $10^p x_j$. The L-PRVP is quadratically constrained due to the inner product of $b(u,l)$ and $y$. While MIQCPs are known to be much more computationally demanding than mixed-integer linear programming, we find that in practice we are able to solve the problem in seconds on real-world tabular datasets. This is because the problem only scales with the number of features and actionability constraints, which are typically small, rather than the number of data points in the data set. %Note that if the LRAP problem is \emph{infeasible}, this certifies that every data point in ${\cal X}$ has recourse.


\subsection{Discrete Setting}

So far, we have shown how to construct a region $B(u,l)$ where all data points have no recourse in the L-PREP. Note that any region $B(u,l)$ that is feasible for the L-PRVP also contains no \textit{integer} data points with recourse, as its a relaxation of the discrete problem. However, it may fail to find regions where there is recourse in the relaxed version of the problem, but no feasible recourse in the discrete problem. In this case, the L-PRVP being infeasible cannot certify that all data points have recourse in the discrete problem.

To extend our approach to the discrete setting, we consider a simple strategy that solves the L-PRVP over all possible values of the discrete variables, which we call scenarios. Note that if we can certify recourse for the entire population on every scenario then we have have certified recourse for the discrete version of the problem. Let ${\cal J}_D$ be the set of discrete variables in the PREP. These can include variables $x_j$, $a_j$, or any auxiliary discrete variables that are needed to enforce certain actionability constraints. 

Let ${\cal S}$ be the set of scenarios, where a scenario $s \in {\cal S}$ corresponds to fixed values for the discrete variables (e.g., $x_1 = 1, x_2 = 2$ for ${\cal J}_D = \{1,2\}$). Note that the set ${\cal S}$ grows exponentially with respect to the number of discrete variables, which may become computationally intractable for large problems. However, we prove in Section \ref{sec:scaling} that under very general constraints and minimal assumptions we can relax many of the discrete variables in the PRVP. Under these new theoretical results, the set of scenarios that the algorithm must consider is incredibly small (e.g., $|{\cal S}| \leq 4$) for real-world datasets considered in prior work \cite{kothari2023prediction}. 

We integrate these scenarios into the PREP MILP formulation (see Appendix \ref{app:prep_form}), giving a revised formulation:
$$
A(s)\mathbf{x} + B(s)\mathbf{a} \leq b(\mathbf{u}, \mathbf{l},s)
$$
where $A, B,$ and $b$ now depend on the scenario $s$. To verify recourse over the entire population, we now need to find a certificate of infeasibility $\mathbf{y}_s$ for all scenarios $s \in {\cal S}$, giving rise to the following MIQCP which captures the original PRVP:
\begin{align}
	\textbf{max}~~&& \sum_d \frac{u_d - l_d}{U_d - L_d} \label{obj:f_size}\\[.1cm]
	\textbf{s.t.}~~&& b(\mathbf{u}, \mathbf{l}, s)^T \mathbf{y}_s &= -1 ~~&& \forall s \in {\cal S} \label{const:f_neg_ray}\\
	&& A(s)^T \mathbf{y}_s &= 0 && \forall s \in {\cal S} \label{const:f_dual_feas_a} \\
	&& B(s)^T \mathbf{y}_s &= 0 && \forall s \in {\cal S}\label{const:f_dual_feas_b} \\
	&& \mathbf{y}_s &\geq 0 && \forall s \in {\cal S}\label{const:f_non_neg_y} \\
	&& \mathbf{L} \leq \mathbf{l} \leq \mathbf{u} &\leq \mathbf{U} && \label{const:f_box_bounds} \\
	&& \mathbf{u}, \mathbf{l} &\in \mathbb{Z}^d \label{const:f_ul_int}
\end{align}

Note that when auditing recourse over a \emph{fixed} region $B(\mathbf{u}, \mathbf{l})$ (i.e., the decision-variant of the problem) we can decompose the PRVP into $|{\cal S}|$ problems (i.e., audit recourse for each scenario independently). If the PRVP is infeasible for any scenario (i.e., there exists an individual without recourse), then the PRVP is infeasible for the fixed region. Otherwise, we can certify recourse for the entire population over the region. However, in the interpretable PRVP (i.e., where we aim to find the largest reason) the problem cannot be decomposed as the box upper and lower bound variables link all the sub-problems. 


%\item Scales badly but in next section we show we can relax almost all the variables.

\subsection{Generating multiple regions}
In practice, it may be beneficial to generate multiple regions of data points without recourse to capture diverse sources of preclusion. Our framework can be easily extended to a sequential setting where we generate new regions, or certify that there are no additional regions without recourse. We do so by adding \textit{no-good cuts} to the RAP that excludes previously discovered regions.

Let $\bar{\mathbf{u}}, \bar{\mathbf{l}}$ be an existing region with no recourse. We add decision variables $\mathbf{z}_{u}, \mathbf{z}_{l} \in \{0, 1\}^d$ that track whether our new region $\mathbf{u}, \mathbf{l}$ is outside the existing region. We can model the no-good cuts that exclude $\bar{\mathbf{u}}, \bar{\mathbf{l}}$ using the following linear constraints:

\begin{align}
	 &u_d \leq \bar{l}_d - 1 + (U_d - \bar{l}_d - 1)(1-z_{ud}) ~~ \forall d \in [d] \label{const:ub}\\
	& l_d \geq \bar{u}_d + 1 + (L_d - \bar{u}_d + 1)(1-z_{ld}) ~~ \forall d \in [d] \label{const:lb}\\
    &\sum_d z_{ud} + z_{ld} \geq 1 \label{const:z_sum} \\
    & \mathbf{z}_{u}, \mathbf{z}_{l} \in \{0, 1\}^d \label{const:z_bin} 
\end{align}

Constraint \eqref{const:ub} checks whether the upper bound for feature $d$ in our new region is less than the lower bound for feature $d$ in the existing region. Note that these constraints are enforced if $z_{ud} = 1$. Constraint \eqref{const:lb} checks an analogous condition for the lower bound of feature d. Constraints \eqref{const:z_sum}-\eqref{const:z_bin} ensure that at least one constraint of type \eqref{const:ub} or \eqref{const:lb} are active. In other words, it ensures that the new region must fall outside the previous region by ensuring that in at least one feature the boxes do not coincide. Note that we can exclude constraints for bounds that are tight with the population bounds (i.e., $u_d = U_d$ or $l_d = L_d$). Given that our procedure tends to generate sparse regions (i.e., regions that change few features from their population upper and lower bounds), these no good-cuts typically add a very small number of binary variables and constraints to the full formulation.

%We can generate a set of regions by repeatedly solving the RAP and cutting off previous regions by adding new constraint blocks \eqref{const:ub}-\eqref{const:z_bin}. Given our assumption that the input data is integer, this procedure can in theory enumerate all possible regions with no recourse. In practice this is only feasible in settings where there are a small number of regions without recourse.


==> deprecated/5_scaling.tex <==
\section{Relaxing Discrete Variables} \label{sec:scaling}
In the preceding section, we showed that we could solve the PRVP with discrete variables by enumerating all scenarios (i.e., fixed values for the discrete variables) and solving a MIQCP over all scenarios. However, this approach scales exponentially with respect to the number of discrete variables in the PREP. In this section we show that under a very broad set of actionability constraints and general assumptions we can relax all the discrete variables in the PREP problem and still certify population-level recourse.

We consider the following set of candidate constraints. We allow these constraints to act on either $x$ variables, $a$ variables, or both. Let $v_j$ represent a set of variables corresponding to feature $j$ (i.e., $x_j, a_j$, or $x_j+a_j$). 

\textbf{K-Hot Constraints:} These constraints capture that the unweighted sum of variables is exactly, at most, or at least $K \in \mathbb{Z}$. Let $J_c$ be the set of variables that participate in a k-hot constraint $c$. As an example, a K-Hot constraint can be represented by:
$$
\sum_{j \in J_c}  \pm~v_j \leq K
$$
Note that this constraint generalizes the popular \emph{one-hot encoding} for categorical variables.


\textbf{Unit Directional Linkage Constraints:} These constraints encode that a unit change in one feature, $v_{j}$ implies a unit change in another feature $v_{k}$. When applied to $\mathbf{x}$ variables it implies that one feature is always greater than or equal to another.
$$
v_{j} \leq v_{k}
$$
This family of constraints can ensure a broad class of non-separable constraints including thermometer encoding, and deterministic causal constraints (e.g., increasing years of account history implies a commensurate increase in Age). 

\textbf{Integer Bound Constraints:} These constraints put an integer upper or lower bounds on a variable. 
$$
L_j \leq  v_j \leq U_j
$$
This simple constraint class encompasses a wide range of separable constraints including monotonicity, actionability, and bounds on the action step size \cite{kothari2023prediction}.

We denote an action set comprised of these constraints as \textit{linear recourse constraints}. Linear recourse constraints encompass a very broad set of actionability constraints considered in previous literature including categorical encodings, thermometer encodings, montonocity, actionability, and action step sizes. This encompasses all the constraints in \citet{ustun2019actionable, russell2019efficient}, and all but 2 of the 100+ constraints used in the experiments in \citet{kothari2023prediction}. We now show that with two additional general assumptions, we can relax all the discrete variables in the PREP.

\begin{assumption}[A1, Informal\label{a1:onehot}] 
All variables participate in at most one $k$-hot constraint.
\end{assumption}

\begin{assumption}[A2, Informal\label{a2:directional_linkage}] 
The set of directional linkage constraints do not imply any relationships between variables participating in k-hot constraints.
\end{assumption}

Under these assumptions, the following result shows that solving the L-PREP is equivalent to solve the PREP. Practically, this means that we can relax all discrete variables in the problem and audit the model using the L-PRVP. 

\begin{theorem}\label{thm:tum}
Under Assumptions \ref{a1:onehot} and \ref{a2:directional_linkage}, the L-PRVP with linear recourse constraints is feasible iff the PRVP is feasible.
\end{theorem}

\textit{Proof Sketch.} At a high-level, we prove this result by showing that the polyhedron defining feasible $x$ and recourse $a$ under linear recourse constraints is \emph{totally unimodular}, which means that all extreme points of the polyhedron are integral. Consequently, a solution to the L-PREP exists if and only if there is at least one solution to the PREP, and by extension the PRVP. For a full proof, and formal definitions of the assumptions please see Appendix X.




==> deprecated/linear_recourse_constraints.tex <==
\textbf{K-Hot Constraints:} These constraints capture that the unweighted sum of variables is exactly, at most, or at least $K \in \mathbb{Z}$. Let $J_i$ be the set of variables that participate in a K-hot constraint $i$. A K-Hot constraint can be written as
$$
\sum_{j \in J_i}  \pm~v_j \leq K.
$$
This constraint generalizes the popular \emph{one-hot encoding} for categorical variables.

\textbf{Unit Directional Linkage Constraints:} These constraints encode that a unit change in one feature, $v_{j}$ implies a unit change in another feature $v_{k}$: 
$$
v_{j} \leq v_{k}.
$$
This constraint on $\mathbf{x}$ variables implies that one feature is always greater than or equal to another.
This family of constraints can ensure a broad class of non-separable constraints (i.e., constraints that act on multiple features) including thermometer encodings, and deterministic causal constraints (e.g., increasing years of account history implies a commensurate increase in Age). 

\textbf{Integer Bound Constraints:} These constraints put an integer upper or lower bound on a variable:
$$
L_j \leq  v_j \leq U_j.
$$
This simple constraint class encompasses a wide range of separable constraints including monotonicity, actionability, and bounds on the action step size \cite{kothari2023prediction}.


==> sections/0_abstract.tex <==

% Recourse is important

% Existing methods can miss recourse, hard to find reason data points don't have recourse, slow if have to check all data points
Machine learning models routinely support or automate decisions that affect individuals -- deciding who receives loans, a job interview, or an organ transparent. In these settings, models can assign \emph{fixed predictions} that individuals cannot change that individuals cannot change. 
%
%Existing methods can only verify recourse exists for individual data points. To verify recourse over an entire population to which a model is being deployed, these individualized procedures need to be run on a dataset sampled from the population which can be computationally demanding, miss out-of-sample instances without recourse, require access to (possibly) sensitive data, or yield uninterpretable results. 
%
In this work, we introduce a approach based on mixed-integer quadratically-constrained programming that can certify that an entire population has recourse under a linear classifier, or identify interpretable regions with no recourse. Our approach handles a broad class of constraints on actions, and runs in a under a second on real-world datasets. 
%
We conduct a comprehensive empirical study of recourse verification on datasets from consumer finance. Our results highlight individualized recourse methods may misleadingly certify recourse for a population and emphasize the importance of population-based approaches.

% Comically long abstract
%Machine learning (ML) is increasingly being used in high stakes domains to decide who receives loans, jobs, or even livers. In these settings, it is critical that ML models offer individuals \textit{recourse}, the ability to change the decision of a model.%, or else they risk precluding access to credit, employment, and healthcare. While we typically want to certify recourse over the population to a which a ML model could be applied, existing methods can only verify recourse on individual data points. Running these procedures on a dataset sampled from the population can be computationally demanding, miss out-of-sample instances without recourse, and yield results that are difficult to interpret for model developers. In this work, we introduce a novel approach that is able to certify whether an entire population has actionable recourse under a linear classifier. Our method leverages a Mixed-Integer Quadratically Constrained Programming model that is able to either certify recourse over the entire population, or generate an interpretable region within the population with no recourse. Our approach handles a broad class of actionability constraints, and runs in a fraction of the time it takes to audit recourse for every data point individually within the population. We conduct a comprehensive empirical study of our approach on datasets from consumer finance. Our results highlight that existing approaches may misleadingly certify recourse for a population, emphasizing the need for tools that audit recourse beyond individual data points.


==> sections/0_abstract_new.tex <==
Machine learning models that assign predictions to people often fail to account for how individuals can change their characteristics. As a result, models can assign \emph{fixed} predictions that preclude individuals from changing their outcome. This work presents a new paradigm to identify fixed predictions by finding \emph{confined regions} of the feature space in which all individuals receive fixed predictions. We develop a method to discover confined regions for linear classifiers using mixed-integer quadratically constrained programming. Our approach certifies recourse for out-of-sample data, provides interpretable descriptions of confined regions, and runs in seconds on real-world datasets. We conduct a comprehensive empirical study of confined regions across diverse applications. Our results highlight that existing pointwise verification methods fail to discover confined regions, while our method provably succeeds. 

==> sections/1_introduction.tex <==
\section{Introduction}

Machine learning is increasingly used in high-stakes settings to decide who receives a loan \citep{hurley2016credit}, a job interview~\citep{bogen2018help}, or an organ transplant~\citep{murgia2023algorithms}. Models predict outcomes using features about individuals, without considering how individuals can change them~\citep[][]{liu2024actionability}. Consequently, models may assign an individual a \emph{fixed prediction} which is not \emph{responsive} to their actions. 

The responsiveness of a model is integral to its safety in settings where predictions map to people. In lending and hiring, fixed predictions may preclude individuals from access to credit and employment. In content moderation, a fixed prediction can ensure that malicious actors are unable to evade detection by manipulating their features. There has been little work that mentions this effect, let alone studies it. Yet fixed predictions arise in practice. Recently, a predictive model used to allocate livers in the United Kingdom was found to precluding all young patients -- no matter how ill -- from receiving a liver transplant~\cite{murgia2023algorithms}. %Despite the gravity of this problem, no existing methods can characterize the set of individuals who receive fixed predictions under a model.

The difficulties in detecting fixed predictions stem from challenges in optimization, interpretability, and data collection. Verifying recourse for a \emph{single individual} is a non-trivial combinatorial problem that requires performing exhaustive search over a subset of the feature space that captures both the model as well as actionability constraints \cite{ustun2019actionable, kothari2023prediction}. Characterizing all fixed predictions represents an even more intensive setting that requires searching over any plausible individual. Moreover, even when individuals without recourse can be identified, it is hard to determine the cause of these fixed predictions \citep{rawal2020algorithmic}. The standard pointwise approach to check model responsiveness \citep[see][]{kothari2023prediction} can only verify recourse for available data, and does not provide guarantees on model responsiveness out-of-sample. In practice, this means that critical issues can only be identified \emph{after} a model has been deployed and it is too late to prevent harms.  %The utility of these point-wise approaches is dependent on access to comprehensive data sets that cover potential model users. However, this is an onerous requirement for external audits where gaining access to a model is easy but getting a representative sample of the population is difficult. For instance, many interpretable medical and criminal justice scoring systems are available publicly~\citep[see e.g.,][]{morrison2022optimized, yamga2023optimized, ribeiro2023use, PennSentence}, but gaining access to a representative dataset is difficult due to privacy concerns. 

%Point-wise approaches to recourse verification also require access to a representative dataset of individuals affected by the model. This requirement is impossible in settings with distribution shift after deployment, and demanding for external audits where gaining access to a model is easy but getting a representative sample of the population is difficult. For instance, many interpretable medical and criminal justice scoring systems are available publicly~\citep[see e.g.,][]{morrison2022optimized, yamga2023optimized, ribeiro2023use, PennSentence}, but gaining access to a representative dataset is difficult due to privacy concerns. Moreover, even when individuals without recourse can be identified during model development, determining the root cause of fixed predictions can be challenging!\citep{rawal2020algorithmic}. 

This work studies a new paradigm in algorithmic recourse that characterizes fixed predictions by verifying recourse over an \emph{entire region} of the feature space (e.g., all plausible job applicants). We develop a method to find confined regions by \emph{Mixed-Integer Quadratically Constrained Programming} (MIQCP) to audit linear classifiers. Our approach can identify \emph{confined regions} (i.e., where all individuals are assigned a fixed prediction) within the feature space, or provide a formal certification of model responsiveness over the entire region. Our approach is robust to distribution shifts, interpretable, and runs in seconds on real-world datasets.  Moreover, our tool can be used without the need for available datasets. This enables practitioners to audit model responsiveness in settings with only model access and a description of the population on which it is being deployed. For instance, many interpretable medical and criminal justice scoring systems are available publicly~\citep[see e.g.,][]{morrison2022optimized,yamga2023optimized,ribeiro2023use, PennSentence}, but gaining access to a representative dataset is difficult due to privacy concerns. 

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/overview_2.pdf}
    \vspace{-2em}
    \caption{Stylized recourse verification problem that aims to find all individuals that are assigned a fixed prediction under a given classifier. The feature space (1) defines all possible feature vectors $\mathbf{x}$. The region of interest (2) is a subset of the feature space representing individuals on which to audit recourse. The action set (3) defines a set of constraints on what actions $\mathbf{a}$ individuals can take to change their prediction under a classifier (4). A confined region (5) is a subset of the region of interest in which all individuals are assigned a fixed prediction, which depends on both the classifier and the action set. In this example, a single confined regions provides an interpretable characterization of all individuals that receive a fixed prediction.}
    \label{fig:summary}
    \vspace{-1em}
\end{figure*}

The main contributions of this work include:
%
\begin{enumerate}[leftmargin=*,itemsep=0pt]
    % Conceptual Contributions
    \item We introduce a new approach to formally verify recourse for linear classifiers 
    over entire regions of the feature space. This tool can be used certify the responsiveness of classifiers beyond data present in a training dataset and can provide stronger guarantees for out-of-sample data. We also present tools to find (or enumerate all) confined regions in the feature space, providing an intuitive tool for model developers to audit and correct problems with model responsiveness.

    % Method Constribution
    \item We develop fast methods that are able to find confined regions via MIQCP. Our approach handles a broad class of actionability constraints, and can verify recourse within seconds on real-world datasets.
    
    % Empirical Contribution
    \item We evaluate our approach on applications in consumer finance, content moderation, and criminal justice. Our results show that point-wise verification approaches fail to verify model responsiveness over regions, emphasizing the need for tools that audit recourse beyond individual data points. We also showcase the ability of our approach to audit model responsiveness in settings with no public datasets via a case-study on the Pennsylvania criminal justice sentencing risk assessment instrument.

    % Software
    %\item We include a Python implementation of our approach that builds upon existing APIs for actionable recourse, allowing practitioners to easily specify complex actionability constraints and audit recourse.
    
\end{enumerate}




==> tables/fico_population_bound_table.tex <==
\begin{tabular}{llll}
\toprule
\textheader{Name} & \textheader{Type} & \textheader{LB} & \textheader{UB} \\
\midrule
\textfn{ExternalRiskEstimate} & $\mathbb{Z}$ & 3 & 9 \\
\textfn{YearsOfAccountHistory} & $\mathbb{Z}$ & 0 & 50 \\
\textfn{AvgYearsInFile} & $\mathbb{Z}$ & 0 & 19 \\
\textfn{MostRecentTradeWithinLastYear} & $\{0,1\}$ & 0 & 1 \\
\textfn{MostRecentTradeWithinLast2Years} & $\{0,1\}$ & 0 & 1 \\
\textfn{AnyDerogatoryComment} & $\{0,1\}$ & 0 & 1 \\
\textfn{AnyTrade120DaysDelq} & $\{0,1\}$ & 0 & 1 \\
\textfn{AnyTrade90DaysDelq} & $\{0,1\}$ & 0 & 1 \\
\textfn{AnyTrade60DaysDelq} & $\{0,1\}$ & 0 & 1 \\
\textfn{AnyTrade30DaysDelq} & $\{0,1\}$ & 0 & 1 \\
\textfn{NoDelqEver} & $\{0,1\}$ & 0 & 1 \\
\textfn{YearsSinceLastDelqTradeLeq1} & $\{0,1\}$ & 0 & 1 \\
\textfn{YearsSinceLastDelqTradeLeq3} & $\{0,1\}$ & 0 & 1 \\
\textfn{YearsSinceLastDelqTradeLeq5} & $\{0,1\}$ & 0 & 1 \\
\textfn{NumInstallTrades} & $\mathbb{Z}$ & 0 & 55 \\
\textfn{NumRevolvingTrades} & $\mathbb{Z}$ & 0 & 85 \\
\textfn{NetFractionInstallBurden} & $\mathbb{Z}$ & 0 & 47 \\
\textfn{NetFractionRevolvingBurden} & $\mathbb{Z}$ & 0 & 23 \\
\textfn{NumBank2NatlTradesWHighUtilizationGeq2} & $\{0,1\}$ & 0 & 1 \\
\bottomrule
\end{tabular}


==> tables/fico_population_constraints.tex <==
\begin{constraints}
\item ThermometerEncoding: Actions on [\textfn{ExternalRiskEstimate$\geq$40}, \textfn{ExternalRiskEstimate$\geq$50}, \textfn{ExternalRiskEstimate$\geq$60}, \textfn{ExternalRiskEstimate$\geq$70}, \textfn{ExternalRiskEstimate$\geq$80}] must preserve thermometer encoding., which can only increase.Actions can only turn on higher-level dummies that are off, where \textfn{ExternalRiskEstimate$\geq$40} is the lowest-level dummy and \textfn{ExternalRiskEstimate$\geq$80} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{YearsSinceLastDelqTrade$\leq$1}, \textfn{YearsSinceLastDelqTrade$\leq$3}, \textfn{YearsSinceLastDelqTrade$\leq$5}] must preserve thermometer encoding., which can only decrease.Actions can only turn off higher-level dummies that are on, where \textfn{YearsSinceLastDelqTrade$\leq$1} is the lowest-level dummy and \textfn{YearsSinceLastDelqTrade$\leq$5} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{MostRecentTradeWithinLast2Years}, \textfn{MostRecentTradeWithinLastYear}] must preserve thermometer encoding.
\item ThermometerEncoding: Actions on [\textfn{AvgYearsInFile$\geq$3}, \textfn{AvgYearsInFile$\geq$5}, \textfn{AvgYearsInFile$\geq$7}] must preserve thermometer encoding., which can only increase.Actions can only turn on higher-level dummies that are off, where \textfn{AvgYearsInFile$\geq$3} is the lowest-level dummy and \textfn{AvgYearsInFile$\geq$7} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{NetFractionRevolvingBurden$\geq$10}, \textfn{NetFractionRevolvingBurden$\geq$20}, \textfn{NetFractionRevolvingBurden$\geq$50}] must preserve thermometer encoding., which can only decrease.Actions can only turn off higher-level dummies that are on, where \textfn{NetFractionRevolvingBurden$\geq$10} is the lowest-level dummy and \textfn{NetFractionRevolvingBurden$\geq$50} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{NetFractionInstallBurden$\geq$10}, \textfn{NetFractionInstallBurden$\geq$20}, \textfn{NetFractionInstallBurden$\geq$50}] must preserve thermometer encoding., which can only decrease.Actions can only turn off higher-level dummies that are on, where \textfn{NetFractionInstallBurden$\geq$10} is the lowest-level dummy and \textfn{NetFractionInstallBurden$\geq$50} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{NumRevolvingTradesWBalance$\geq$2}, \textfn{NumRevolvingTradesWBalance$\geq$3}, \textfn{NumRevolvingTradesWBalance$\geq$5}, \textfn{NumRevolvingTradesWBalance$\geq$7}] must preserve thermometer encoding., which can only decrease.Actions can only turn off higher-level dummies that are on, where \textfn{NumRevolvingTradesWBalance$\geq$2} is the lowest-level dummy and \textfn{NumRevolvingTradesWBalance$\geq$7} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{NumRevolvingTrades$\geq$2}, \textfn{NumRevolvingTrades$\geq$3}, \textfn{NumRevolvingTrades$\geq$5}, \textfn{NumRevolvingTrades$\geq$7}] must preserve thermometer encoding., which can only decrease.Actions can only turn off higher-level dummies that are on, where \textfn{NumRevolvingTrades$\geq$2} is the lowest-level dummy and \textfn{NumRevolvingTrades$\geq$7} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{NumInstallTradesWBalance$\geq$2}, \textfn{NumInstallTradesWBalance$\geq$3}, \textfn{NumInstallTradesWBalance$\geq$5}, \textfn{NumInstallTradesWBalance$\geq$7}] must preserve thermometer encoding., which can only decrease.Actions can only turn off higher-level dummies that are on, where \textfn{NumInstallTradesWBalance$\geq$2} is the lowest-level dummy and \textfn{NumInstallTradesWBalance$\geq$7} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{NumInstallTrades$\geq$2}, \textfn{NumInstallTrades$\geq$3}, \textfn{NumInstallTrades$\geq$5}, \textfn{NumInstallTrades$\geq$7}] must preserve thermometer encoding., which can only decrease.Actions can only turn off higher-level dummies that are on, where \textfn{NumInstallTrades$\geq$2} is the lowest-level dummy and \textfn{NumInstallTrades$\geq$7} is the highest-level-dummy.
\end{constraints}

==> tables/givemecredit_population_bound_table.tex <==
\begin{tabular}{llll}
\toprule
\textheader{Name} & \textheader{Type} & \textheader{LB} & \textheader{UB} \\
\midrule
\textfn{Age} & $\mathbb{Z}$ & 21 & 103 \\
\textfn{NumberOfDependents} & $\mathbb{Z}$ & 0 & 20 \\
\textfn{DebtRatio$\geq$1} & $\{0,1\}$ & 0 & 1 \\
\textfn{MonthlyIncome$\geq$3K} & $\{0,1\}$ & 0 & 1 \\
\textfn{MonthlyIncome$\geq$5K} & $\{0,1\}$ & 0 & 1 \\
\textfn{MonthlyIncome$\geq$10K} & $\{0,1\}$ & 0 & 1 \\
\textfn{CreditLineUtilization$\geq$10} & $\{0,1\}$ & 0 & 1 \\
\textfn{CreditLineUtilization$\geq$20} & $\{0,1\}$ & 0 & 1 \\
\textfn{CreditLineUtilization$\geq$50} & $\{0,1\}$ & 0 & 1 \\
\textfn{CreditLineUtilization$\geq$70} & $\{0,1\}$ & 0 & 1 \\
\textfn{CreditLineUtilization$\geq$100} & $\{0,1\}$ & 0 & 1 \\
\textfn{AnyRealEstateLoans} & $\{0,1\}$ & 0 & 1 \\
\textfn{MultipleRealEstateLoans} & $\{0,1\}$ & 0 & 1 \\
\textfn{AnyCreditLinesAndLoans} & $\{0,1\}$ & 0 & 1 \\
\textfn{MultipleCreditLinesAndLoans} & $\{0,1\}$ & 0 & 1 \\
\textfn{HistoryOfLatePayment} & $\{0,1\}$ & 0 & 1 \\
\textfn{HistoryOfDelinquency} & $\{0,1\}$ & 0 & 1 \\
\bottomrule
\end{tabular}


==> tables/givemecredit_population_constraints.tex <==
\begin{constraints}
\item ThermometerEncoding: Actions on [\textfn{MonthlyIncome$\geq$3K}, \textfn{MonthlyIncome$\geq$5K}, \textfn{MonthlyIncome$\geq$10K}] must preserve thermometer encoding., which can only increase.Actions can only turn on higher-level dummies that are off, where \textfn{MonthlyIncome$\geq$3K} is the lowest-level dummy and \textfn{MonthlyIncome$\geq$10K} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{CreditLineUtilization$\geq$10}, \textfn{CreditLineUtilization$\geq$20}, \textfn{CreditLineUtilization$\geq$50}, \textfn{CreditLineUtilization$\geq$70}, \textfn{CreditLineUtilization$\geq$100}] must preserve thermometer encoding., which can only decrease.Actions can only turn off higher-level dummies that are on, where \textfn{CreditLineUtilization$\geq$10} is the lowest-level dummy and \textfn{CreditLineUtilization$\geq$100} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{AnyRealEstateLoans}, \textfn{MultipleRealEstateLoans}] must preserve thermometer encoding., which can only decrease.Actions can only turn off higher-level dummies that are on, where \textfn{AnyRealEstateLoans} is the lowest-level dummy and \textfn{MultipleRealEstateLoans} is the highest-level-dummy.
\item ThermometerEncoding: Actions on [\textfn{AnyCreditLinesAndLoans}, \textfn{MultipleCreditLinesAndLoans}] must preserve thermometer encoding., which can only decrease.Actions can only turn off higher-level dummies that are on, where \textfn{AnyCreditLinesAndLoans} is the lowest-level dummy and \textfn{MultipleCreditLinesAndLoans} is the highest-level-dummy.
\end{constraints}

==> tables/results_table.tex <==
\begin{tabular}{llllll}
\
\textbf{Dataset} & \textbf{Metrics} & \us{} & \baseline{Data Sample} & \baseline{Region Sample} & \baseline{Classifier Extremes} \\
\midrule
\multirow[c]{7}{*}{\ficoinfo{}} & Certifies Responsive & 54.2\% & --- & --- & --- \\
 & Outputs Responsive & 54.2\% & 91.6\% & 66.5\% & 71.0\% \\
 & \sublevel~Blindspot & \textbf{0.0\%} & \textcolor{\pitfall}{37.4\%} & \textcolor{\pitfall}{12.3\%} & \textcolor{\pitfall}{16.8\%} \\
 & Certifies Static & 0.0\% & --- & --- & --- \\
 & Outputs Static & 0.0\% & 0.6\% & 0.0\% & 0.0\% \\
 & \sublevel~Loophole & \textbf{0.0\%} & \textcolor{\pitfall}{0.6\%} & \textbf{0.0\%} & \textbf{0.0\%} \\
 & Comp. Time (s) & 4.67(3.6) & 0.05(0.0) & 0.74(0.1) & 0.02(0.0) \\
\cmidrule{1-6}
\multirow[c]{7}{*}{\givemecreditinfo{}} & Certifies Responsive & 60.1\% & --- & --- & --- \\
 & Outputs Responsive & 60.1\% & 72.2\% & 60.1\% & 62.9\% \\
 & \sublevel~Blindspot & \textbf{0.0\%} & \textcolor{\pitfall}{12.0\%} & \textbf{0.0\%} & \textcolor{\pitfall}{2.8\%} \\
 & Certifies Static & 18.3\% & --- & --- & --- \\
 & Outputs Static & 18.3\% & 19.4\% & 19.2\% & 19.2\% \\
 & \sublevel~Loophole & \textbf{0.0\%} & \textcolor{\pitfall}{1.1\%} & \textcolor{\pitfall}{0.8\%} & \textcolor{\pitfall}{0.8\%} \\
 & Comp. Time (s) & 0.13(0.1) & 0.02(0.1) & 0.32(0.1) & 0.01(0.0) \\
\cmidrule{1-6}
\multirow[c]{7}{*}{\twitterbotinfo{}} & Certifies Responsive & 25.0\% & --- & --- & --- \\
 & Outputs Responsive & 25.0\% & 40.0\% & 25.0\% & 25.0\% \\
 & \sublevel~Blindspot & \textbf{0.0\%} & \textcolor{\pitfall}{15.0\%} & \textbf{0.0\%} & \textbf{0.0\%} \\
 & Certifies Static & 5.0\% & --- & --- & --- \\
 & Outputs Static & 5.0\% & 25.0\% & 25.0\% & 25.0\% \\
 & \sublevel~Loophole & \textbf{0.0\%} & \textcolor{\pitfall}{20.0\%} & \textcolor{\pitfall}{20.0\%} & \textcolor{\pitfall}{20.0\%} \\
 & Comp. Time (s) & 0.07(0.2) & 0.02(0.0) & 0.36(0.1) & 0.01(0.0) \\

\end{tabular}


==> tables/results_table_bu.tex <==
\begin{tabular}{@{}llllll@{}}
 & & & \multicolumn{3}{c}{\baseline{PointWise}} \\ \cmidrule{4-6}
\textbf{Dataset} & \textbf{Metrics} & \us{} & \baseline{Data} & \baseline{Region} & \baseline{Score} \\
\toprule
\multirow[c]{7}{*}{\ficoinfo{}} & Certifies Responsive & 54.2\% & --- & --- & --- \\
 & Outputs Responsive & 54.2\% & 91.6\% & 66.5\% & 71.0\% \\
 & \sublevel~Blindspot & \textbf{0.0\%} & \textcolor{\pitfall}{37.4\%} & \textcolor{\pitfall}{12.3\%} & \textcolor{\pitfall}{16.8\%} \\
 & Certifies Static & 0.0\% & --- & --- & --- \\
 & Outputs Static & 0.0\% & 0.6\% & 0.0\% & 0.0\% \\
 & \sublevel~Loophole & \textbf{0.0\%} & \textcolor{\pitfall}{0.6\%} & \textbf{0.0\%} & \textbf{0.0\%} \\
 %& Comp. Time (s) & 4.67(3.6) & 0.05(0.0) & 0.74(0.1) & 0.02(0.0) \\

\cmidrule{1-6}

\multirow[c]{7}{*}{\givemecreditinfo{}} & Certifies Responsive & 60.1\% & --- & --- & --- \\
 & Outputs Responsive & 60.1\% & 72.2\% & 60.1\% & 62.9\% \\
 & \sublevel~Blindspot & \textbf{0.0\%} & \textcolor{\pitfall}{12.0\%} & \textbf{0.0\%} & \textcolor{\pitfall}{2.8\%} \\
 & Certifies Static & 18.3\% & --- & --- & --- \\
 & Outputs Static & 18.3\% & 19.4\% & 19.2\% & 19.2\% \\
 & \sublevel~Loophole & \textbf{0.0\%} & \textcolor{\pitfall}{1.1\%} & \textcolor{\pitfall}{0.8\%} & \textcolor{\pitfall}{0.8\%} \\
 %& Comp. Time (s) & 0.13(0.1) & 0.02(0.1) & 0.32(0.1) & 0.01(0.0) \\
\cmidrule{1-6}

\multirow[c]{7}{*}{\twitterbotinfo{}} & Certifies Responsive & 25.0\% & --- & --- & --- \\
 & Outputs Responsive & 25.0\% & 40.0\% & 25.0\% & 25.0\% \\
 & \sublevel~Blindspot & \textbf{0.0\%} & \textcolor{\pitfall}{15.0\%} & \textbf{0.0\%} & \textbf{0.0\%} \\
 & Certifies Static & 5.0\% & --- & --- & --- \\
 & Outputs Static & 5.0\% & 25.0\% & 25.0\% & 25.0\% \\
 & \sublevel~Loophole & \textbf{0.0\%} & \textcolor{\pitfall}{20.0\%} & \textcolor{\pitfall}{20.0\%} & \textcolor{\pitfall}{20.0\%} \\
% & Comp. Time (s) & 0.07(0.2) & 0.02(0.0) & 0.36(0.1) & 0.01(0.0) \\

\cmidrule{1-6}
\end{tabular}

==> tables/twitterbot_population_bound_table.tex <==
\begin{tabular}{llll}
\toprule
\textheader{Name} & \textheader{Type} & \textheader{LB} & \textheader{UB} \\
\midrule
\textfn{SourceAutomation} & $\{0,1\}$ & 0 & 1 \\
\textfn{SourceOther} & $\{0,1\}$ & 0 & 1 \\
\textfn{SourceBranding} & $\{0,1\}$ & 0 & 1 \\
\textfn{SourceMobile} & $\{0,1\}$ & 0 & 1 \\
\textfn{SourceWeb} & $\{0,1\}$ & 0 & 1 \\
\textfn{SourceApp} & $\{0,1\}$ & 0 & 1 \\
\textfn{FollowerFriendRatio$\geq$1} & $\{0,1\}$ & 0 & 1 \\
\textfn{FollowerFriendRatio$\geq$10} & $\{0,1\}$ & 0 & 1 \\
\textfn{FollowerFriendRatio$\geq$100} & $\{0,1\}$ & 0 & 1 \\
\textfn{FollowerFriendRatio$\geq$1000} & $\{0,1\}$ & 0 & 1 \\
\textfn{FollowerFriendRatio$\geq$10000} & $\{0,1\}$ & 0 & 1 \\
\textfn{FollowerFriendRatio$\geq$100000} & $\{0,1\}$ & 0 & 1 \\
\textfn{AgeOfAccountInDays$\geq$365} & $\{0,1\}$ & 0 & 1 \\
\textfn{AgeOfAccountInDays$\geq$730} & $\{0,1\}$ & 0 & 1 \\
\textfn{UserReplied$\geq$10} & $\{0,1\}$ & 0 & 1 \\
\textfn{UserReplied$\geq$100} & $\{0,1\}$ & 0 & 1 \\
\textfn{UserFavourited$\geq$1000} & $\{0,1\}$ & 0 & 1 \\
\textfn{UserFavourited$\geq$10000} & $\{0,1\}$ & 0 & 1 \\
\textfn{UserRetweeted$\geq$1} & $\{0,1\}$ & 0 & 1 \\
\textfn{UserRetweeted$\geq$10} & $\{0,1\}$ & 0 & 1 \\
\textfn{UserRetweeted$\geq$100} & $\{0,1\}$ & 0 & 1 \\
\bottomrule
\end{tabular}


==> tables/twitterbot_population_constraints.tex <==
\begin{constraints}
\item ThermometerEncoding: Actions on [\textfn{FollowerFriendRatio$\geq$1}, \textfn{FollowerFriendRatio$\geq$10}, \textfn{FollowerFriendRatio$\geq$100}, \textfn{FollowerFriendRatio$\geq$1000}, \textfn{FollowerFriendRatio$\geq$10000}, \textfn{FollowerFriendRatio$\geq$100000}] must preserve thermometer encoding.
\item ThermometerEncoding: Actions on [\textfn{AgeOfAccountInDays$\geq$365}, \textfn{AgeOfAccountInDays$\geq$730}] must preserve thermometer encoding.
\item ThermometerEncoding: Actions on [\textfn{UserReplied$\geq$10}, \textfn{UserReplied$\geq$100}] must preserve thermometer encoding.
\item ThermometerEncoding: Actions on [\textfn{UserFavourited$\geq$1000}, \textfn{UserFavourited$\geq$10000}] must preserve thermometer encoding.
\item ThermometerEncoding: Actions on [\textfn{UserRetweeted$\geq$1}, \textfn{UserRetweeted$\geq$10}, \textfn{UserRetweeted$\geq$100}] must preserve thermometer encoding.
\end{constraints}
